Local Binary Pattern Networks

Memory and computation efficient deep learning architec- tures are crucial to continued proliferation of machine learning capabili- ties to new platforms and systems. Binarization of operations in convo- lutional neural networks has shown promising results in reducing model size and computing efficiency. In this paper, we tackle the problem us- ing a strategy different from the existing literature by proposing local binary pattern networks or LBPNet, that is able to learn and perform binary operations in an end-to-end fashion. LBPNet1 uses local binary comparisons and random projection in place of conventional convolu- tion (or approximation of convolution) operations. These operations can be implemented efficiently on different platforms including direct hard- ware implementation. We applied LBPNet and its variants on standard benchmarks. The results are promising across benchmarks while provid- ing an important means to improve memory and speed efficiency that is particularly suited for small footprint devices and hardware accelerators.

==> backup.tex <==
%%% Abstract %%%
%Convolutional neural networks (CNN) have achieved excellent performance in image classification tasks. However, the state-of-the-art CNN models rely on powerful parallel computing machines too much because of the intense high-precision computations and heavy memory accesses. In this paper, we propose local binary pattern network, LBPNet, to replace multiplication and addition with comparison and memory allocation to alleviate the resource demands of CNN models. More specifically, we propose both the forward and backward propagations of LBPNet. Our model has been verified on MNIST and CIFAR-10 datasets and achieved $99.00\%$ and $87\%$ accuracy, respectively.

%In this paper, we explore a new direction, local binary pattern networks (LBPNet), that is able to learn and perform binary operations in an end-to-end fashion from scratch. In LBPNet, the basic operations are no longer convolution, which is in distinction to the existing approaches in which either binarization is performed to approximate convolution or convolution is used to approximate the local binary operations. The basic building blocks in LBPNet include local binary comparison (to replace convolution) and random projection (to replace $1\times 1$ convolution), both resulting in efficient logic operations. We applied LBPNet and its variants on standard benchmarks and observed modest results. LBPNet has its unique architecture demonstrating desirable properties as an alternative to convolution with memory and speed efficiency suited for hardware accelerator.

%%% Experiment Setup %%%
\begin{table}
\vspace{-3mm}
%\begin{wraptable}{r}{0.35\linewidth} \small
%\vspace{-12mm}
\small
\centering
\caption{The performance of the classifier on three datasets.}
\vspace{-1mm}
\scalebox{0.9}{
\begin{tabular}{||l|r||}
\hline
Dataset          &  Error \\  \hline
MNIST            & 24.22\% \\
SVHN             & 77.78\% \\
CIFAR-10         & 65.91\% \\
\hline
\end{tabular}
}
\label{tab:classifier}
\vspace{-4mm}
%\end{wraptable}
\end{table}

%\vspace{-3mm}
%\subsection{Ablation Study}
%\label{sec:ablation}
%\vspace{-1mm}
% 1. Starting from a canonical model
% 2. gradually replace convolutional layer with LBP layer
% 3. Try different number of kernels
% 4. Results and Discussion

%\begin{wraptable}{r}{0.5\linewidth} \small
%\vspace{-11mm}
%\small
%\centering
%\caption{Comparison between LBCNN and LBPNet on CIFAR-10 for an ablation study.}
%\vspace{+2mm}
%\scalebox{0.9}{
%\begin{tabular}{||c|l|rrr||}
%\hline
%\multirow{2}{*}{}&  &\multirow{2}{*}{Error} & Size    & Latency \\ 
%                 &  &                       & (Byte)  & (cycles)                 \\ \hline
%\multicolumn{2}{||c|}{CNN (10-layer)}   &  8.39\% & 31.19M & 1.426G \\ \hline
%\multirow{2}{*}{1L} & LBCNN             & 18.82\% & 30.55M & 1.239G \\
%                    & LBPNet & 11.62\% & 30.68M & 1.417G \\ \hline
%\multirow{2}{*}{2L} & LBCNN             & 18.76\% & 30.27M & 1.080G \\
%                    & LBPNet & 13.79\% & 30.15M & 1.058G \\ \hline
%\multirow{2}{*}{3L} & LBCNN             & 19.17\% & 29.04M & 0.920G \\
%                    & LBPNet & 17.13\% & 28.90M & 0.982G \\ \hline
%\multirow{2}{*}{4L} & LBCNN             & 21.08\% & 22.55M & 0.761G \\
%                    & LBPNet & 27.92\% & 24.34M & 0.907G \\
%\hline
%\end{tabular}
%}
%\label{tab:ablation_cifar10}
%\vspace{-4mm}
%\end{wraptable}
%In this section, we conduct ablation experiments for LBCNN and LBPNets(RDP) on CIFAR-10.
%Starting from the $10$-layer baseline CNNs for CIFAR-10 in previous section, we gradually replace convolutional layers with LBP layers and LBCNN layers.
%The target convolutional layer for ablation are \#1, \#3, \#5 and \#8.
%The results of ablation on CIFAR-10 are listed in Table~\ref{tab:ablation_cifar10}.% and Fig.~\ref{fig:ablation}.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.6\columnwidth]{fig/ablation.png}
% 	\caption{The result of the ablation experiment.}
%     \label{fig:ablation}
% \vspace{-6mm}
% \end{figure}

%As shown in Table~\ref{tab:ablation_cifar10}, the error rates are rising when more layers of convolutions are being replaced. LBPNet outperforms LBCNN when fewer convolution layers are being replaced. Gradually, LBCNN starts to outperform LBPNet.
%Fig.~\ref{fig:ablation} also indicates that LBP layer is more sensitive to the spatial size of input feature maps.
%Our explanation is the limiting area of LBPNet's pattern is $5$-by-$5$.
%Although a $4$-by-$4$ incoming feature map is padded with two rings of zeros, the sampled pixels are too sparse to extract helpful features.

